Falsification Of The Atmospheric CO2 Greenhouse Effects Within The Frame Of Physics

The atmospheric greenhouse effect, an idea that many authors trace back to the traditional works of Fourier (1824), Tyndall (1861), and Arrhenius (1896), and which is still supported in global climatology, essentially describes a fictitious mechanism, in which a planetary atmosphere acts as a heat pump driven by an environment that is radiatively interacting with but radiatively equilibrated to the atmospheric system. According to the second law of thermodynamics such a planetary machine can never exist. Nevertheless, in almost all texts of global climatology and in a widespread secondary literature it is taken for granted that such mechanism is real and stands on a firm scientific foundation. In this paper the popular conjecture is analyzed and the underlying physical principles are clarified. By showing that (a) there are no common physical laws between the warming phenomenon in glass houses and the fictitious atmospheric greenhouse effects, (b) there are no calculations to determine an average surface temperature of a planet, (c) the frequently mentioned difference of 33 degrees Celsius is a meaningless number calculated wrongly, (d) the formulas of cavity radiation are used inappropriately, (e) the assumption of a radiative balance is unphysical, (f) thermal conductivity and friction must not be set to zero, the atmospheric greenhouse conjecture is falsified.

==> GerlichTscheuschner2007a_001_settings_TeX4ht_.tex <==
\newcommand{\TschCurrentVersion}{Version 4.0 (January 6, 2009)}
\newcommand{\TschFirstVersion}{replaces Version 1.0 (July 7, 2007) and later}
%
\newcommand{\TschReferencesPageMode}{FromTo}
\newcommand{\TschStyle}{TeX4ht}
\newcommand{\TschStyles}{arXivOrTeX4ht}
\newcommand{\TschSpace}{\ }
%
\newcommand{\TschGerlich}{Gerhard Gerlich}
\newcommand{\TschTscheuschner}{Ralf D. Tscheuschner}
%
\newcommand{\TschAuthors}{\TschGerlich\ and \TschTscheuschner}
%
\newcommand{\TschTitleLineA}{Falsification Of}
\newcommand{\TschTitleLineB}{The Atmospheric CO$_2$ Greenhouse Effects}
\newcommand{\TschTitleLineBbf}{The Atmospheric
                               CO$_{\mbox{{\small\textbf{2}}}}$
                               Greenhouse Effects}
\newcommand{\TschTitleLineC}{Within The Frame Of Physics}
\newcommand{\TschTitleLineCdots}{$\dots$}
%
\newcommand{\TschTitle}{\TschTitleLineA\ \TschTitleLineB\ \TschTitleLineCdots}


==> GerlichTscheuschner2007a_006_abstract_txt_.tex <==
Gerhard Gerlich, Ralf D. Tscheuschner

Falsification Of The Atmospheric CO2 Greenhouse Effects Within The Frame Of Physics

The atmospheric greenhouse effect, an idea that many authors trace
back to the traditional works of Fourier (1824), Tyndall (1861), and
Arrhenius (1896), and which is still supported in global
climatology, essentially describes a fictitious mechanism, in which
a planetary atmosphere acts as a heat pump driven by an environment
that is radiatively interacting with but radiatively equilibrated to
the atmospheric system. According to the second law of
thermodynamics such a planetary machine can never exist.
Nevertheless, in almost all texts of global climatology and in a
widespread secondary literature it is taken for granted that such
mechanism is real and stands on a firm scientific foundation. In
this paper the popular conjecture is analyzed and the underlying
physical principles are clarified. By showing that (a) there are no
common physical laws between the warming phenomenon in glass houses
and the fictitious atmospheric greenhouse effects, (b) there are no
calculations to determine an average surface temperature of a
planet, (c) the frequently mentioned difference of 33 degrees
Celsius is a meaningless number calculated wrongly, (d) the formulas
of cavity radiation are used inappropriately, (e) the assumption of
a radiative balance is unphysical, (f) thermal conductivity and
friction must not be set to zero, the atmospheric greenhouse
conjecture is falsified.


==> GerlichTscheuschner2007a_010_keywords_.tex <==
\keywords{Greenhouse Effect; Gibbs Thermodynamics; Radiation Theory.} 


==> GerlichTscheuschner2007a_099_toc_.tex <==
\tableofcontents 
